Linear Item-Item Model with Neural Knowledge for Session-based Recommendation

Session-based recommendation (SBR) aims to predict users' subsequent actions by modeling short-term interactions within sessions. Existing neural models primarily focus on capturing complex dependencies for sequential item transitions. As an alternative solution, linear item-item models mainly identify strong co-occurrence patterns across items and support faster inference speed. Although each paradigm has been actively studied in SBR, their fundamental differences in capturing item relationships and how to bridge these distinct modeling paradigms effectively remain unexplored. In this paper, we propose a novel SBR model, namely Linear Item-Item model with Neural Knowledge (LINK), which integrates both types of knowledge into a unified linear framework. Specifically, we design two specialized components of LINK: (i) Linear knowledge-enhanced Item-item Similarity model (LIS), which refines the item similarity correlation via self-distillation, and (ii) Neural knowledge-enhanced Item-item Transition model (NIT), which seamlessly incorporates complicated neural knowledge distilled from the off-the-shelf neural model. Extensive experiments demonstrate that LINK outperforms state-of-the-art linear SBR models across six real-world datasets, achieving improvements of up to 14.78% and 11.04% in Recall@20 and MRR@20 while showing up to 813x fewer inference FLOPs. Our code is available at https://github.com/jin530/LINK.

==> Figures_tex/Fig_co_occur_performance.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=1\linewidth]{Figures/fig_digi_comparaitive_performance.png}
\caption{Performance over various session groups for Diginetica. Each session is categorized into Head(Top20\%)/Tail(Bottom80\%), HighSim($>$0.5)/LowSim($\le$0.5) based on the popularity of the last item and the normalized co-occurrence score of the last item and the target item.}\label{fig:co_occur_performance}
\end{figure*}


==> Figures_tex/Fig_co_occur_similarity_1col.tex <==
\begin{figure}
\centering
\includegraphics[width=1.0\linewidth]{Figures/fig_digi_comparative_sk.png}
\caption{
\mj{
Distribution of item similarity scores over co-occurrences for consecutive item pairs (former item $\rightarrow$ latter item). The color indicates the popularity of the former item. For simplicity, we linearly scale the similarity into $[0, 1]$ and normalize co-occurrence by the popularity of the former item. Data points represent all consecutive item pairs extracted from validation sessions in the Diginetica dataset. 
} 
}\label{fig:co_occur}
\Description{}{}
% \vspace{-3mm}
\end{figure}
% (a) CORE is one of the state-of-the-art neural SBR models, while (b) SLIST and (c) SWalk are linear SBR models. 
% Item-item similarity scores between two consecutive items (source $\rightarrow$ target) in the validation sessions in the Diginetica dataset. 
% For simplicity, we linearly scale the similarities into $[0, 1]$.
% The color indicates the popularity of the source item.

==> Figures_tex/Fig_extend_r.tex <==




\begin{figure*}[t]\small
\centering
\includegraphics[width=1.0\linewidth]{Figures/fig_hyper_r.png}
\caption{Performance of LINK over varied extended ratio $r$.}\label{fig:exp_extend_r}
\vspace{-3mm}
\end{figure*}




==> Figures_tex/Fig_flops.tex <==
\begin{figure}
\includegraphics[width=1.0\linewidth]{Figures/digi_flops_recall.png} 
\caption{Performance comparison over the Recall@20 and the log-scaled number of floating point operations (FLOPs) for inference on the Diginetica dataset. The numbers in parentheses indicate the relative FLOPs compared to LINK.}\label{fig:exp_flops}
\vspace{-3mm}
\Description{}{}
\end{figure}


\iffalse
% -- Two columns figure --

\begin{figure*}
\begin{tabular}{cc}
\includegraphics[width=0.4\linewidth]{Figures/digi_flops_recall.png} 
& \includegraphics[width=0.4\linewidth]{Figures/yc_flops_recall.png}  \\
(a) Diginetica & (b) Yoochoose
\end{tabular}
\caption{Performance comparison over the Recall@20 and the number of floating point operations for inference. The numbers in parentheses indicate the multiple of FLOPs compared to LINK.}\label{fig:exp_flops}
\Description{}{}
\end{figure*}
% The square marker indicates a linear model. The circle, triangle, and diamond markers indicate RNN-, GNN-, and transformer-based neural models, respectively.




\fi

==> Figures_tex/Fig_session_length.tex <==
\begin{figure*}[t]\small
\centering
\includegraphics[width=1.0\linewidth]{Figures/fig_length.png}
\caption{Performance comparison of SBR models over varying session lengths. Sessions are divided into six groups depending on session length. The square marker indicates a linear model, and the triangle marker indicates a neural model.}\label{fig:exp_session_length}
\vspace{-3mm}
\end{figure*}



==> Figures_tex/Fig_teacher_beta.tex <==
\begin{figure*}[t]\small
\centering
\includegraphics[width=1.0\linewidth]{Figures/fig_hyper_lambda.png}
\caption{Performance of LINK over varying regularization coefficient $\lambda$.}\label{fig:exp_teacher_beta}
\vspace{-3mm}
\end{figure*}






==> Figures_tex/Fig_teacher_tau.tex <==
\begin{figure*}[t]\small
\centering
\includegraphics[width=1.0\linewidth]{Figures/fig_hyper_tau.png}
\caption{Performance of LINK over varying temperature $\tau$.}\label{fig:exp_teacher_tau}
\vspace{-3mm}
\end{figure*}


\iffalse

\begin{figure}[t]
\centering
\begin{tabular}{ccc}
\includegraphics[width=0.3\textwidth]{Figures/fig_length_diginetica.png}  &
\includegraphics[width=0.3\textwidth]{Figures/fig_length_diginetica.png}  & 
\includegraphics[width=0.3\textwidth]{Figures/fig_length_diginetica.png}  
\\
(a) Diginetica & (b) Retailrocket & (c) Yoochoose \\
\end{tabular}
\caption{Performance of LINK over varied temperature $\tau$.}\label{fig:exp_teacher_tau}
\vspace{-3mm}
\end{figure}


\fi

==> Figures_tex/Fig_weight_alpha.tex <==
\begin{figure*}[t]\small
\centering
\includegraphics[width=1.0\linewidth]{Figures/fig_hyper_alpha.png}
\caption{Performance of LINK over varied $\alpha$.}\label{fig:exp_weight_alpha}
\vspace{-3mm}
\end{figure*}


\iffalse
\begin{figure}[t]
\centering
\begin{tabular}{ccc}
\includegraphics[width=0.3\textwidth]{Figures/fig_length_diginetica.png}  &
\includegraphics[width=0.3\textwidth]{Figures/fig_length_diginetica.png}  & 
\includegraphics[width=0.3\textwidth]{Figures/fig_length_diginetica.png}  
\\
(a) Diginetica & (b) Retailrocket & (c) Yoochoose \\
\end{tabular}
\caption{Performance of LINK over varied $\alpha$.}\label{fig:exp_weight_alpha}
\vspace{-3mm}
\end{figure}

\fi

==> Table/tab_efficiency.tex <==
\begin{table}[]
\caption{The number of floating point operations and runtime (in seconds) for inference of LINK and DNN-based models. Gain indicates how fast LINK is compared to the best competing model. Runtime for DNN models was measured on GPU with batch size 512, while that for LINK on both CPU and GPU.}
\label{tab:exp_efficiency}
\centering
\begin{tabular}{c|rr|rr|rr}
\toprule
\multirow{2}{*}{Model} & \multicolumn{2}{c|}{Diginetica} & \multicolumn{2}{c|}{Retailrocket} & \multicolumn{2}{c}{Yoochoose} \\
 & \multicolumn{1}{c}{GFLOPs} & \multicolumn{1}{c|}{Time (sec)} & \multicolumn{1}{c}{GFLOPs} & \multicolumn{1}{c|}{Time (sec)} & \multicolumn{1}{c}{GFLOPs} & \multicolumn{1}{c}{Time (sec)} \\ \midrule
CORE & 53429.73 & 0.54 & 51319.58 & 0.07 & 253016.86 & 0.16  \\
MSGIFSR & 0000.0 & 10.06 & 0000.0 & 11.43 & 0000.0 & 12.62  \\
SCL & 0000.0 & 1.88 & 0000.0 & 2.07 & 0000.0 & 2.61  \\ \midrule
LINK (GPU) & 6.58 & 0.84 & 7.70 & 0.81 & 6.60 & 0.33 \\ 
LINK (CPU) & 6.57 & 28.64 & 7.69 & 51.09 & 6.59 & 38.02 \\ \midrule
Gain & 0000.0x & 00.0x & 0000.0x & 00.0x & 0000.0x & 00.0x \\ \bottomrule
\end{tabular}
\end{table}

==> Table/tab_length_1.tex <==
\begin{table}[]
\caption{Performance (Recall@20) of various SBR models for sessions with length 1 on Diginetica.}
\label{tab:exp_length_1}
\centering
\setlength{\tabcolsep}{2.3pt} 
\begin{tabular}{c|cccc|cc}
\hline
\multirow{2}{*}{Diginetica} & \multicolumn{4}{c|}{Neural Models} & \multicolumn{2}{c}{Linear Models} \\ \cline{2-7} 
 & GCEGNN~\citep{WangWCLMQ20GCEGNN} & CORE~\citep{hou2022core} & MSGIFSR~\citep{Guo0SZWBZ22MSGIFSR} & SCL~\cite{ShiWL24SCL} & SLIST~\citep{ChoiKLSL21SLIST} & SWalk~\citep{ChoiKLSL22S-Walk} \\ \hline
Sessions ($L=1$) & 50.39 & \textbf{52.63} & 51.63 & 51.66 & 46.45 & {49.31} \\
All sessions & 50.43 & 52.97 & 52.64 & 51.89 & 49.81 & {51.19} \\ \hline
\end{tabular}
\end{table}


% \begin{table}[]
% \caption{Performance of various SBR models for sessions with length 1 on Diginetica.}
% \label{tab:exp_length_1}
% \centering
% \begin{tabular}{c|cccc|ccc}
% \hline
% \multirow{2}{*}{Diginetica} & \multicolumn{4}{c|}{Neural Models} & \multicolumn{3}{c}{Linear Models} \\ \cline{2-8} 
%  & GCEGNN & CORE & MSGIFSR & SCL & SLIST & \multicolumn{1}{c|}{SWalk} & \textbf{LINK} \\ \hline
% Sessions w/ L=1 & 50.39 & 52.63 & 51.63 & 51.66 & 46.45 & \multicolumn{1}{c|}{49.31} & 52.21 \\
% All sessions & 50.43 & 52.97 & 52.64 & 51.89 & 49.81 & \multicolumn{1}{c|}{51.19} & 53.33 \\ \hline
% \end{tabular}
% \end{table}

==> Table/tab_optimal_hyperparmeter.tex <==
\begin{table}[]
\centering
\caption{Optimal hyperparameters of LINK for each dataset.}\label{tab:optimal_hyper}
\begin{tabular}{c|cccccc}
\toprule
Dataset & $\alpha$ & $\beta$ & $\lambda$ & $\tau$ & $\delta_{\text{pos}}$ & $\delta_{\text{inf}}$ \\
\midrule
Diginetica & 0.9 & 1.0 & 10$^2$ & 0.1 & 1.0 & 4.0 \\
Retailrocket & 0.9 & 0.9 & 10$^2$ & 0.1 & 1.0 & 4.0 \\
Yoochoose & 0.5 & 1.0 & 10$^3$ & 0.1 & 1.0 & 1.0 \\
Tmall & 0.9 & 1.0 & 10$^3$ & 0.05 & 1.0 & 4.0 \\
Dressipi & 0.9 & 0.5 & 10$^2$ & 0.1 & 1.0 & 4.0 \\
LastFM & 0.9 & 1.0 & 10$^2$ & 0.1 & 1.0 & 8.0 \\
% \midrule
% Beauty & 0 & 100 & - & 1.0 & 1.0 \\
% Toys & 0 & 200 & - & 1.0 & 1.0 \\
% Sports & 0 & 1000 & - & 1.0 & 1.0 \\
% Yelp & 0.7 & 200 & 1 & 2.0 & 2.0 \\
\bottomrule
\end{tabular}
\end{table}



==> Table/tab_overall_performance_ttest.tex <==
\begin{table*} \small
\centering
% \setlength{\tabcolsep}{1.9pt} 
\renewcommand{\arraystretch}{1}
\caption{Performance comparison of our proposed model and competing models. Gain indicates how much better the proposed model is than the best linear model. The best model is marked in \textbf{bold}, and the second-best model is \ul{underlined}. }\label{tab:exp_all_ttest}
\begin{tabular}{ccccccc}
\toprule
\multicolumn{1}{c|}{\multirow{2}{*}{Model}} & \multicolumn{2}{c|}{Diginetica} & \multicolumn{2}{c|}{Retailrocket} & \multicolumn{2}{c}{Yoochoose} \\
\multicolumn{1}{c|}{} & R@20 & \multicolumn{1}{c|}{M@20} & R@20 & \multicolumn{1}{c|}{M@20} & R@20 & M@20 \\ \midrule
\multicolumn{7}{c}{\textit{Neural Models}} \\ \midrule
\multicolumn{1}{c|}{GRU4Rec} & 47.19 \scriptsize $\pm$ 0.19 & \multicolumn{1}{c|}{15.73 \scriptsize $\pm$ 0.04} & 57.79 \scriptsize $\pm$ 0.07 & \multicolumn{1}{c|}{34.87 \scriptsize $\pm$ 0.13} & 61.16 \scriptsize $\pm$ 0.26 & 27.19 \scriptsize $\pm$ 0.15 \\
\multicolumn{1}{c|}{NARM} & 48.09 \scriptsize $\pm$ 0.18 & \multicolumn{1}{c|}{16.01 \scriptsize $\pm$ 0.09} & 59.21 \scriptsize $\pm$ 0.18 & \multicolumn{1}{c|}{35.61 \scriptsize $\pm$ 0.12} & 62.43 \scriptsize $\pm$ 0.21 & 28.25 \scriptsize $\pm$ 0.12 \\
\multicolumn{1}{c|}{STAMP} & 44.25 \scriptsize $\pm$ 0.10 & \multicolumn{1}{c|}{14.84 \scriptsize $\pm$ 0.05} & 53.86 \scriptsize $\pm$ 0.18 & \multicolumn{1}{c|}{31.89 \scriptsize $\pm$ 0.14} & 60.50 \scriptsize $\pm$ 0.33 & 27.87 \scriptsize $\pm$ 0.10 \\
\multicolumn{1}{c|}{SASRec} & 35.73 \scriptsize $\pm$ 7.13 & \multicolumn{1}{c|}{13.14 \scriptsize $\pm$ 2.10} & 58.93 \scriptsize $\pm$ 0.13 & \multicolumn{1}{c|}{35.32 \scriptsize $\pm$ 0.08} & 62.47 \scriptsize $\pm$ 0.35 & 27.77 \scriptsize $\pm$ 0.14 \\
\multicolumn{1}{c|}{SR-GNN} & 48.41 \scriptsize $\pm$ 0.16 & \multicolumn{1}{c|}{16.45 \scriptsize $\pm$ 0.12} & 58.72 \scriptsize $\pm$ 0.10 & \multicolumn{1}{c|}{35.49 \scriptsize $\pm$ 0.07} & 62.10 \scriptsize $\pm$ 0.32 & 28.17 \scriptsize $\pm$ 0.11 \\
\multicolumn{1}{c|}{NISER+} & 50.80 \scriptsize $\pm$ 0.25 & \multicolumn{1}{c|}{17.91 \scriptsize $\pm$ 0.16} & 60.70 \scriptsize $\pm$ 0.12 & \multicolumn{1}{c|}{37.95 \scriptsize $\pm$ 0.12} & 63.33 \scriptsize $\pm$ 0.26 & 29.02 \scriptsize $\pm$ 0.08 \\
\multicolumn{1}{c|}{GC-SAN} & 49.94 \scriptsize $\pm$ 0.17 & \multicolumn{1}{c|}{17.39 \scriptsize $\pm$ 0.08} & 60.04 \scriptsize $\pm$ 0.04 & \multicolumn{1}{c|}{36.23 \scriptsize $\pm$ 0.11} & 62.70 \scriptsize $\pm$ 0.33 & 28.68 \scriptsize $\pm$ 0.14 \\
\multicolumn{1}{c|}{LESSR} & 48.45 \scriptsize $\pm$ 0.16 & \multicolumn{1}{c|}{16.33 \scriptsize $\pm$ 0.21} & 57.75 \scriptsize $\pm$ 1.18 & \multicolumn{1}{c|}{36.35 \scriptsize $\pm$ 0.20} & 62.51 \scriptsize $\pm$ 0.45 & 28.25 \scriptsize $\pm$ 0.21 \\
\multicolumn{1}{c|}{GCE-GNN} & 50.46 \scriptsize $\pm$ 0.06 & \multicolumn{1}{c|}{17.71 \scriptsize $\pm$ 0.09} & 60.42 \scriptsize $\pm$ 0.16 & \multicolumn{1}{c|}{35.70 \scriptsize $\pm$ 0.05} & 63.31 \scriptsize $\pm$ 0.13 & 28.95 \scriptsize $\pm$ 0.13 \\
\multicolumn{1}{c|}{SGNN-HN} & 50.58 \scriptsize $\pm$ 0.10 & \multicolumn{1}{c|}{17.10 \scriptsize $\pm$ 0.03} & 58.64 \scriptsize $\pm$ 0.57 & \multicolumn{1}{c|}{35.31 \scriptsize $\pm$ 0.09} & 61.99 \scriptsize $\pm$ 0.31 & 28.23 \scriptsize $\pm$ 0.05 \\
\multicolumn{1}{c|}{DSAN} & 51.64 \scriptsize $\pm$ 0.17 & \multicolumn{1}{c|}{18.32 \scriptsize $\pm$ 0.04} & 61.00 \scriptsize $\pm$ 0.48 & \multicolumn{1}{c|}{38.76 \scriptsize $\pm$ 0.06} & 63.44 \scriptsize $\pm$ 0.18 & \ul{29.08} \scriptsize $\pm$ 0.14 \\
\multicolumn{1}{c|}{CORE} & \ul{52.87} \scriptsize $\pm$ 0.09 & \multicolumn{1}{c|}{18.59 \scriptsize $\pm$ 0.05} & 62.00 \scriptsize $\pm$ 0.07 & \multicolumn{1}{c|}{38.17 \scriptsize $\pm$ 0.13} & 64.57 \scriptsize $\pm$ 0.05 & 28.35 \scriptsize $\pm$ 0.02 \\
\multicolumn{1}{c|}{MSGIFSR} & 52.54 \scriptsize $\pm$ 0.16 & \multicolumn{1}{c|}{\ul{19.06} \scriptsize $\pm$ 0.08} & \ul{62.67} \scriptsize $\pm$ 0.11 & \multicolumn{1}{c|}{\textbf{39.08 \scriptsize $\pm$ 0.05}} & \ul{64.81} \scriptsize $\pm$ 0.09 & \textbf{30.41} \scriptsize $\pm$ 0.05 \\
\multicolumn{1}{c|}{SCL} & 52.03 \scriptsize $\pm$ 0.14 & \multicolumn{1}{c|}{18.84 \scriptsize $\pm$ 0.09} & 60.12 \scriptsize $\pm$ 0.11 & \multicolumn{1}{c|}{37.88 \scriptsize $\pm$ 0.13} & 63.47 \scriptsize $\pm$ 0.17 & \ul{29.07} \scriptsize $\pm$ 0.11 \\ \midrule
\multicolumn{7}{c}{\textit{Linear Models}} \\ \midrule
\multicolumn{1}{c|}{SLIST} & 49.81 & \multicolumn{1}{c|}{18.45} & 60.10 & \multicolumn{1}{c|}{37.69} & 63.32 & 28.30 \\
\multicolumn{1}{c|}{S-Walk} & 51.19 & \multicolumn{1}{c|}{18.76} & 61.31 & \multicolumn{1}{c|}{38.79} & 63.72 & 27.61 \\ \midrule
\multicolumn{1}{c|}{LINK} & \textbf{53.62} & \multicolumn{1}{c|}{\textbf{19.22}} & \textbf{62.74} & \multicolumn{1}{c|}{\ul{38.97}} & \textbf{64.90} & 28.82 \\ \midrule
\multicolumn{1}{c|}{Gain (\%)} & 4.75 & \multicolumn{1}{c|}{2.45} & 2.33 & \multicolumn{1}{c|}{0.46} & 1.85 & 1.84 \\ 
\midrule
\midrule
\end{tabular}

\begin{tabular}{ccccccc}

\multicolumn{1}{c|}{\multirow{2}{*}{Model}} & \multicolumn{2}{c|}{Tmall} & \multicolumn{2}{c|}{Dressipi} & \multicolumn{2}{c}{LastFM} \\
\multicolumn{1}{c|}{} & R@20 & \multicolumn{1}{c|}{M@20} & R@20 & \multicolumn{1}{c|}{M@20} & R@20 & M@20 \\ \midrule
\multicolumn{7}{c}{\textit{Neural Models}} \\ \midrule
\multicolumn{1}{c|}{GRU4Rec} & 33.87 \scriptsize $\pm$ 0.15 & \multicolumn{1}{c|}{23.37 \scriptsize $\pm$ 0.28} & 35.33 \scriptsize $\pm$ 0.31 & \multicolumn{1}{c|}{13.74 \scriptsize $\pm$ 0.14} & 20.88 \scriptsize $\pm$ 0.11 & 7.21 \scriptsize $\pm$ 0.07 \\
\multicolumn{1}{c|}{NARM} & 35.55 \scriptsize $\pm$ 0.27 & \multicolumn{1}{c|}{24.58 \scriptsize $\pm$ 0.18} & 37.40 \scriptsize $\pm$ 0.21 & \multicolumn{1}{c|}{14.80 \scriptsize $\pm$ 0.08} & 20.91 \scriptsize $\pm$ 0.19 & 7.34 \scriptsize $\pm$ 0.03 \\
\multicolumn{1}{c|}{STAMP} & 22.79 \scriptsize $\pm$ 2.10 & \multicolumn{1}{c|}{15.67 \scriptsize $\pm$ 1.11} & 36.17 \scriptsize $\pm$ 0.23 & \multicolumn{1}{c|}{14.56 \scriptsize $\pm$ 0.14} & 19.93 \scriptsize $\pm$ 0.29 & 7.40 \scriptsize $\pm$ 0.07 \\
\multicolumn{1}{c|}{SASRec} & 36.32 \scriptsize $\pm$ 0.16 & \multicolumn{1}{c|}{25.66 \scriptsize $\pm$ 0.10} & 32.71 \scriptsize $\pm$ 0.39 & \multicolumn{1}{c|}{12.28 \scriptsize $\pm$ 0.23} & 14.49 \scriptsize $\pm$ 0.77 & 4.15 \scriptsize $\pm$ 0.29 \\
\multicolumn{1}{c|}{SR-GNN} & 34.78 \scriptsize $\pm$ 0.31 & \multicolumn{1}{c|}{24.82 \scriptsize $\pm$ 0.49} & 35.62 \scriptsize $\pm$ 0.23 & \multicolumn{1}{c|}{14.14 \scriptsize $\pm$ 0.16} & 21.45 \scriptsize $\pm$ 0.20 & 8.63 \scriptsize $\pm$ 0.08 \\
\multicolumn{1}{c|}{NISER+} & 40.17 \scriptsize $\pm$ 0.10 & \multicolumn{1}{c|}{29.16 \scriptsize $\pm$ 0.04} & 37.97 \scriptsize $\pm$ 0.10 & \multicolumn{1}{c|}{15.13 \scriptsize $\pm$ 0.10} & 22.15 \scriptsize $\pm$ 0.09 & \ul{8.64} \scriptsize $\pm$ 0.02 \\
\multicolumn{1}{c|}{GC-SAN} & 36.60 \scriptsize $\pm$ 0.08 & \multicolumn{1}{c|}{24.65 \scriptsize $\pm$ 0.09} & 37.62 \scriptsize $\pm$ 0.12 & \multicolumn{1}{c|}{14.97 \scriptsize $\pm$ 0.03} & 21.83 \scriptsize $\pm$ 0.11 & 8.54 \scriptsize $\pm$ 0.02 \\
\multicolumn{1}{c|}{LESSR} & 33.97 \scriptsize $\pm$ 0.22 & \multicolumn{1}{c|}{24.40 \scriptsize $\pm$ 0.18} & 36.84 \scriptsize $\pm$ 0.29 & \multicolumn{1}{c|}{14.30 \scriptsize $\pm$ 0.06} & 21.93 \scriptsize $\pm$ 0.15 & 8.56 \scriptsize $\pm$ 0.06 \\
\multicolumn{1}{c|}{GCE-GNN} & 36.25 \scriptsize $\pm$ 0.21 & \multicolumn{1}{c|}{26.73 \scriptsize $\pm$ 0.13} & 37.23 \scriptsize $\pm$ 0.24 & \multicolumn{1}{c|}{14.97 \scriptsize $\pm$ 0.06} & 22.75 \scriptsize $\pm$ 0.13 & 8.35 \scriptsize $\pm$ 0.03 \\
\multicolumn{1}{c|}{SGNN-HN} & 39.66 \scriptsize $\pm$ 0.33 & \multicolumn{1}{c|}{23.62 \scriptsize $\pm$ 0.16} & 38.39 \scriptsize $\pm$ 0.18 & \multicolumn{1}{c|}{15.05 \scriptsize $\pm$ 0.08} & 22.72 \scriptsize $\pm$ 0.10 & 7.72 \scriptsize $\pm$ 0.04 \\
\multicolumn{1}{c|}{DSAN} & 42.87 \scriptsize $\pm$ 0.25 & \multicolumn{1}{c|}{30.94 \scriptsize $\pm$ 0.04} & 37.19 \scriptsize $\pm$ 0.14 & \multicolumn{1}{c|}{14.86 \scriptsize $\pm$ 0.07} & 22.49 \scriptsize $\pm$ 0.09 & 7.92 \scriptsize $\pm$ 0.06 \\
\multicolumn{1}{c|}{CORE} & 44.88 \scriptsize $\pm$ 0.10 & \multicolumn{1}{c|}{\ul{31.49} \scriptsize $\pm$ 0.04} & 38.33 \scriptsize $\pm$ 0.13 & \multicolumn{1}{c|}{15.70 \scriptsize $\pm$ 0.03} & 22.82 \scriptsize $\pm$ 0.13 & 8.16 \scriptsize $\pm$ 0.04 \\
\multicolumn{1}{c|}{MSGIFSR} & \ul{53.07} \scriptsize $\pm$ 0.05 & \multicolumn{1}{c|}{29.20 \scriptsize $\pm$ 0.14} & \ul{40.33} \scriptsize $\pm$ 0.10 & \multicolumn{1}{c|}{16.11 \scriptsize $\pm$ 0.06} & \ul{25.00} \scriptsize $\pm$ 0.10 & \textbf{10.17} \scriptsize $\pm$ 0.04 \\
\multicolumn{1}{c|}{SCL} & 38.55 \scriptsize $\pm$ 0.30 & \multicolumn{1}{c|}{28.33 \scriptsize $\pm$ 0.13} & 38.08 \scriptsize $\pm$ 0.07 & \multicolumn{1}{c|}{15.29 \scriptsize $\pm$ 0.06} & 22.20 \scriptsize $\pm$ 1.72 & 7.93 \scriptsize $\pm$ 1.00 \\  \midrule
\multicolumn{7}{c}{\textit{Linear Models}} \\ \midrule
\multicolumn{1}{c|}{SLIST} & 47.43 & \multicolumn{1}{c|}{28.93} & 40.20 & \multicolumn{1}{c|}{16.13} & 24.63 & 7.73 \\
\multicolumn{1}{c|}{S-Walk} & 48.77 & \multicolumn{1}{c|}{29.52} & 39.80 & \multicolumn{1}{c|}{\ul{16.19}} & 24.84 & 7.70 \\  \midrule
\multicolumn{1}{c|}{LINK} & \textbf{55.98} & \multicolumn{1}{c|}{\textbf{32.78}} & \textbf{41.39} & \multicolumn{1}{c|}{\textbf{16.38}} & \textbf{25.14} & 7.97 \\ \midrule
\multicolumn{1}{c|}{Gain (\%)} & 14.78 & \multicolumn{1}{c|}{11.04} & 2.96 & \multicolumn{1}{c|}{1.17} & 1.21 & 3.10 \\ 
\bottomrule
\end{tabular}

\end{table*}




==> Table/tab_rebuttal_performance_setup.tex <==
\begin{table} \small
\centering
\caption{Performance for Diginetica over different experimental setups. In GCE-GNN setup, the model is trained on the training and validation sets and iteratively tested on the test set for each epoch. }\label{tab:rebuttal_performance_by_setup}
% \begin{tabular}{c|cc|cc}
\begin{tabular}{c|P{0.7cm}P{0.7cm}|P{0.7cm}P{0.7cm}}
\hline
\multirow{2}{*}{Model} & \multicolumn{2}{c|}{Our setup} & \multicolumn{2}{c}{GCE-GNN setup} \\
 & R@20 & M@20 & R@20 & M@20 \\ \hline
CORE & 52.87 & 18.59 & 54.72 & 18.88 \\
SR-GNN & 48.41 & 16.45 & 52.46 & 18.62 \\
GCE-GNN & 50.46 & 17.71 & 53.51 & 18.9 \\
GCE-GNN* & - & - & 54.22 & 19.04 \\
LINK & \textbf{53.62} & \textbf{19.22} & \textbf{55.21} & \textbf{19.46} \\ \hline
\end{tabular}
\end{table}

==> Table/tab_rebuttal_pruning.tex <==
\begin{table} \small
\centering
\caption{Performance of LINK by applying pruning techniques. LINK achieves high accuracy even if it only retains some important parameters.}\label{tab:rebuttal_pruning}
\vspace{-3mm}
\begin{tabular}{c|cc|c}
\toprule
Pruning ratio & \begin{tabular}[c]{@{}c@{}}Random value\\ Recall@20\end{tabular} & \begin{tabular}[c]{@{}c@{}}Highest value\\ R@20\end{tabular} & Param. \\

\midrule
0.02\% & 0.10 & 48.35 & 0.43M \\
0.1\% & 0.28 & 53.55 & 1.8M \\
0.2\% & 0.61 & 53.63 & 4.3M \\
1\% & 2.46 & 53.61 & 18M \\
10\% & 15.04 & 53.62 & 183M \\
100\% & 53.62 & 53.62 & 1837M \\
\bottomrule
\end{tabular}
\end{table}

==> Table/tab_rebuttal_training_time.tex <==
\begin{table} \small
\centering
\caption{Performance, training time, and number of parameters for Diginetica.}\label{tab:training_time}
\begin{tabular}{cccc}
\toprule
\multicolumn{1}{c|}{Model} & \multicolumn{1}{c|}{R@20} & Train & Param. \\ \midrule
\multicolumn{4}{c}{Neural Model} \\ \midrule
\multicolumn{1}{c|}{CORE} & \multicolumn{1}{c|}{52.87} & 858s & 4.5M \\
\multicolumn{1}{c|}{CORE-large} & \multicolumn{1}{c|}{52.47} & 2,072s & 51M \\
\multicolumn{1}{c|}{MSGIFSR} & \multicolumn{1}{c|}{52.54} & 12,527s & 5.0M \\ \midrule
\multicolumn{4}{c}{Linear Model} \\ \midrule
\multicolumn{1}{c|}{SLIST} & \multicolumn{1}{c|}{49.81} & 430s & 1,837M \\
\multicolumn{1}{c|}{SWalk} & \multicolumn{1}{c|}{51.19} & 2,664s & 1,837M \\ \midrule
\multicolumn{1}{c|}{LINK (CORE)} & \multicolumn{1}{c|}{53.62} & \multicolumn{1}{c}{1,814s} & 1,837M \\
\multicolumn{1}{c|}{LINK (MSGIFSR)} & \multicolumn{1}{c|}{52.27} & \multicolumn{1}{c}{13,548s} & 1,837M \\
\multicolumn{1}{c|}{LINK (CORE, Prune)} & \multicolumn{1}{c|}{\textbf{53.63}} & \multicolumn{1}{c}{1,839s} & 4.3M \\ \bottomrule    
\end{tabular}
\end{table}

==> Table/tab_sr_performance_ttest.tex <==
\begin{table*} \small
\centering
% \setlength{\tabcolsep}{2.5pt} 
% \renewcommand{\arraystretch}{1}
\caption{Performance comparison on sequential datasets. Gain indicates how much better the proposed model is than SLIST~\cite{ChoiKLSL21SLIST}. The best model is marked in \textbf{bold}, and the second-best model is \ul{underlined}. }\label{tab:exp_seqrec_ttest}

\begin{tabular}{c|ccc|ccc}
\toprule
\multirow{2}{*}{Model} & \multicolumn{3}{c|}{Beauty} & \multicolumn{3}{c}{Toys} \\
 & R@20 & M@20 & N@20 & R@20 & M@20 & N@20 \\
\midrule
CORE    & 10.78 \scriptsize $\pm$ 0.19 & 1.87 \scriptsize $\pm$ 0.06 & 3.79 \scriptsize $\pm$ 0.09 & 11.47 \scriptsize $\pm$ 0.10  & 2.02 \scriptsize $\pm$ 0.08 & 4.07 \scriptsize $\pm$ 0.09 \\
MSGIFSR & 11.43 \scriptsize $\pm$ 0.15 & \ul{4.34} \scriptsize $\pm$ 0.05 & \ul{5.89} \scriptsize $\pm$ 0.05 & 9.68 \scriptsize $\pm$ 0.14  & 3.95 \scriptsize $\pm$ 0.08 & 5.20 \scriptsize $\pm$ 0.08  \\
SASRec  & 11.88 \scriptsize $\pm$ 0.06 & 3.16 \scriptsize $\pm$ 0.05 & 5.09 \scriptsize $\pm$ 0.05 & 12.12 \scriptsize $\pm$ 0.09 & 3.13 \scriptsize $\pm$ 0.06 & 5.13 \scriptsize $\pm$ 0.05 \\
DuoRec  & 12.21 \scriptsize $\pm$ 0.27 & 3.45 \scriptsize $\pm$ 0.04 & 5.37 \scriptsize $\pm$ 0.09 & 12.83 \scriptsize $\pm$ 0.08 & 3.62 \scriptsize $\pm$ 0.02 & 5.67 \scriptsize $\pm$ 0.02 \\
FEARec  & 12.38 \scriptsize $\pm$ 0.20  & 3.43 \scriptsize $\pm$ 0.07 & 5.39 \scriptsize $\pm$ 0.08 & \ul{13.06} \scriptsize $\pm$ 0.18 & 3.67 \scriptsize $\pm$ 0.06 & 5.76 \scriptsize $\pm$ 0.09 \\
BSARec  & \textbf{12.63} \scriptsize $\pm$ 0.03 & 3.35 \scriptsize $\pm$ 0.04 & 5.39 \scriptsize $\pm$ 0.03 & 12.88 \scriptsize $\pm$ 0.10  & 3.58 \scriptsize $\pm$ 0.16 & 5.62 \scriptsize $\pm$ 0.10  \\
SLIST   & 10.53 & 4.26 & 5.64 & 11.44 & \ul{5.15} & \ul{6.55} \\
\midrule
LINK    & \ul{12.52} & \textbf{4.44} & \textbf{6.20} & \textbf{13.15} & \textbf{5.46} & \textbf{7.16} \\
\midrule
Gain (\%)  & 18.94 & 4.13 & 10.00 & 14.95 & 6.02 & 9.25 \\
\midrule
\midrule
% \bottomrule
\end{tabular}

\begin{tabular}{c|ccc|ccc}
% \toprule
\multirow{2}{*}{Model} & \multicolumn{3}{c|}{Sports} & \multicolumn{3}{c}{Yelp} \\
 & R@20 & M@20 & N@20 & R@20 & M@20 & N@20 \\
\midrule
CORE    & 6.25 \scriptsize $\pm$ 0.23  & 1.19 \scriptsize $\pm$ 0.09 & 2.28 \scriptsize $\pm$ 0.09 & \ul{11.41} \scriptsize $\pm$ 0.12 & 3.44 \scriptsize $\pm$ 0.02 & \ul{5.17} \scriptsize $\pm$ 0.02 \\
MSGIFSR & 5.47 \scriptsize $\pm$ 0.09  & 1.79 \scriptsize $\pm$ 0.05 & 2.58 \scriptsize $\pm$ 0.05 & 7.90 \scriptsize $\pm$ 0.12   & 2.39 \scriptsize $\pm$ 0.09 & 3.59 \scriptsize $\pm$ 0.09 \\
SASRec  & 6.98 \scriptsize $\pm$ 0.12  & 1.63 \scriptsize $\pm$ 0.06 & 2.81 \scriptsize $\pm$ 0.06 & 8.58 \scriptsize $\pm$ 0.14  & 3.28 \scriptsize $\pm$ 0.03 & 4.42 \scriptsize $\pm$ 0.05 \\
DuoRec  & 7.29 \scriptsize $\pm$ 0.16  & 1.90 \scriptsize $\pm$ 0.05  & 3.08 \scriptsize $\pm$ 0.05 & 9.21 \scriptsize $\pm$ 0.07  & 3.33 \scriptsize $\pm$ 0.04 & 4.60 \scriptsize $\pm$ 0.05  \\
FEARec  & 7.35 \scriptsize $\pm$ 0.23  & 1.90 \scriptsize $\pm$ 0.06  & 3.09 \scriptsize $\pm$ 0.06 & 9.09 \scriptsize $\pm$ 0.03  & 3.26 \scriptsize $\pm$ 0.02 & 4.52 \scriptsize $\pm$ 0.01 \\
BSARec  & \ul{7.78} \scriptsize $\pm$ 0.08  & 1.80 \scriptsize $\pm$ 0.05  & 3.11 \scriptsize $\pm$ 0.05 & 10.09 \scriptsize $\pm$ 0.24 & \ul{3.56} \scriptsize $\pm$ 0.04 & 4.97 \scriptsize $\pm$ 0.07 \\
SLIST   & 6.91 & \ul{2.65} & \ul{3.59} & 9.01 & 3.53 & 4.76 \\
\midrule
LINK    & \textbf{8.17} & \textbf{2.87} & \textbf{4.03} & \textbf{11.67} & \textbf{4.01} & \textbf{5.69} \\
\midrule
Gain (\%)   & 18.21 & 8.23 & 12.14 & 29.48 & 13.65 & 19.50 \\
\bottomrule
\end{tabular}

\end{table*}



==> Table/tab_various_teacher.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]\small
\caption{Performance of LINK with different teacher models.}
\label{tab:exp_various_teacher}
\centering
\begin{tabular}{c|cc|cc|cc}
\toprule
\multirow{2}{*}{Model} & \multicolumn{2}{c|}{Diginetica} & \multicolumn{2}{c|}{Retailrocket} & \multicolumn{2}{c}{Yoochoose} \\
 & R@20 & M@20 & R@20 & M@20 & R@20 & M@20 \\ \midrule
SLIST & 49.81 & 18.45 & 57.40 & 36.06 & 63.32 & 28.30 \\
SWalk & 51.19 & 18.76 & 61.31 & 38.79 & 63.72 & 27.61 \\ \midrule
% LINK (w/ NARM) & 49.36 & 18.05 & 61.61 & 36.72 & 63.13 & 29.07 \\
LINK (w/ CORE~\cite{hou2022core}) & 53.58 & 19.22 & 62.68 & 38.89 & 64.86 & 28.97 \\
LINK (w/ MSGIFSR~\cite{Guo0SZWBZ22MSGIFSR}) & 52.04 & 18.86 & 62.69 & 38.85 & 63.81 & 29.28 \\
LINK (w/ SCL~\cite{ShiWL24SCL})  & 52.49 & 19.04 & 61.62 & 38.73 & 63.09 & 29.11 \\ \bottomrule
\end{tabular}
\end{table}



\iffalse  
\begin{table}[]
\caption{Performance of LINK with different teacher models.}
\label{tab:exp_various_teacher}
\centering
\begin{tabular}{c|ll|ll|ll}
\toprule
\multirow{2}{*}{Model} & \multicolumn{2}{c|}{Diginetica} & \multicolumn{2}{c|}{Retailrocket} & \multicolumn{2}{c}{Yoochoose} \\
 & \multicolumn{1}{c}{R@20} & \multicolumn{1}{c|}{M@20} & \multicolumn{1}{c}{R@20} & \multicolumn{1}{c|}{M@20} & \multicolumn{1}{c}{R@20} & \multicolumn{1}{c}{M@20} \\ \midrule
NARM & 48.35 & 16.01 & 59.39 & 35.68 & 62.57 & 28.34 \\
\& LINK & 48.64 & 16.77 & 61.61 & 36.72 & 63.22 & 28.35 \\ \midrule
MSGIFSR & 52.63 & 19.08 & 62.75 & 38.99 & 64.71 & 30.44 \\
\& LINK& 52.04 & 18.86 & 62.69 & 38.85 & 63.81 & 29.28 \\ \midrule
SCL & 51.84 & 18.84 & 60.45 & 37.79 & 63.52 & 29.29 \\
\& LINK & 52.38 & 19.00 & 61.85 & 38.64 & 64.21 & 28.80 \\ \midrule
MSGIFSR (logit) & 52.37 & 18.17 & 61.96 & 37.37 & 64.40 & 29.79 \\
\& LINK & 49.83 & 17.71 & 59.87 & 36.28 & 64.31 & 29.30 \\ \midrule
SCL (cosine) & 51.93 & 18.83 & 60.35 & 37.80 & 63.52 & 29.25 \\
\& LINK & 52.55 & 18.99 & 59.96 & 37.16 & 64.01 & 29.15  \\ \midrule
CORE & 52.97 & 18.63 & 62.08 & 38.22 & 64.62 & 28.33 \\
\& LINK & 53.58 & 19.22 & 62.68 & 38.89 & 64.86 & 28.97 \\
\bottomrule
\end{tabular}
\end{table}
\fi
